Motion Planning Diffusion: Learning and Planning of Robot Motions with Diffusion Models

Learning priors on trajectory distributions can help accelerate robot motion planning optimization. Given previously successful plans, learning trajectory generative models as priors for a new planning problem is highly desirable. Prior works propose several ways on utilizing this prior to bootstrapping the motion planning problem. Either sampling the prior for initializations or using the prior distribution in a maximum-a-posterior formulation for trajectory optimization. In this work, we propose learning diffusion models as priors. We then can sample directly from the posterior trajectory distribution conditioned on task goals, by leveraging the inverse denoising process of diffusion models. Furthermore, diffusion has been recently shown to effectively encode data multimodality in high-dimensional settings, which is particularly well-suited for large trajectory dataset. To demonstrate our method efficacy, we compare our proposed method - Motion Planning Diffusion - against several baselines in simulated planar robot and 7-dof robot arm manipulator environments. To assess the generalization capabilities of our method, we test it in environments with previously unseen obstacles. Our experiments show that diffusion models are strong priors to encode high-dimensional trajectory distributions of robot motions.

==> bib_old.bib.tex <==
@InProceedings{pmlr-vR4-attias03a,
  title = 	 {Planning by Probabilistic Inference},
  author =       {Attias, Hagai},
  booktitle = 	 {Proceedings of the Ninth International Workshop on Artificial Intelligence and Statistics},
  pages = 	 {9--16},
  year = 	 {2003},
  editor = 	 {Bishop, Christopher M. and Frey, Brendan J.},
  volume = 	 {R4},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {03--06 Jan},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/r4/attias03a/attias03a.pdf},
  url = 	 {https://proceedings.mlr.press/r4/attias03a.html},
  abstract = 	 {This paper presents and demonstrates a new approach to the problem of planning under uncertainty. Actions are treated as hidden variables, with their own prior distributions, in a probabilistic generative model involving actions and states. Planning is done by computing the posterior distribution over actions, conditioned on reaching the goal state within a specified number of steps. Under the new formulation, the toolbox of inference techniques be brought to bear on the planning problem. This paper focuses on problems with discrete actions and states, and discusses some extensions.},
  note =         {Reissued by PMLR on 01 April 2021.}
}


@inproceedings{janner2022diffuser,
  title = {Planning with Diffusion for Flexible Behavior Synthesis},
  author = {Michael Janner and Yilun Du and Joshua Tenenbaum and Sergey Levine},
  booktitle = {International Conference on Machine Learning},
  year = {2022},
}

@inproceedings{
  song2021scorebased,
  title={Score-Based Generative Modeling through Stochastic Differential Equations},
  author={Yang Song and Jascha Sohl-Dickstein and Diederik P Kingma and Abhishek Kumar and Stefano Ermon and Ben Poole},
  booktitle={International Conference on Learning Representations},
  year={2021},
  url={https://openreview.net/forum?id=PxTIG12RRHS}
}

@misc{rombach2021highresolution,
      title={High-Resolution Image Synthesis with Latent Diffusion Models}, 
      author={Robin Rombach and Andreas Blattmann and Dominik Lorenz and Patrick Esser and Björn Ommer},
      year={2021},
      eprint={2112.10752},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@article{neal2022mcmchamiltonian,
author = {Neal, Radford},
year = {2012},
month = {06},
pages = {},
title = {MCMC using Hamiltonian dynamics},
journal = {Handbook of Markov Chain Monte Carlo},
doi = {10.1201/b10905-6}
}



@inproceedings{song2019generativemodeling,
  author    = {Yang Song and
               Stefano Ermon},
  editor    = {Hanna M. Wallach and
               Hugo Larochelle and
               Alina Beygelzimer and
               Florence d'Alch{\'{e}}{-}Buc and
               Emily B. Fox and
               Roman Garnett},
  title     = {Generative Modeling by Estimating Gradients of the Data Distribution},
  booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
               on Neural Information Processing Systems 2019, NeurIPS 2019, December
               8-14, 2019, Vancouver, BC, Canada},
  pages     = {11895--11907},
  year      = {2019},
  url       = {https://proceedings.neurips.cc/paper/2019/hash/3001ef257407d5a371a96dcd947c7d93-Abstract.html},
  timestamp = {Mon, 16 May 2022 15:41:51 +0200},
  biburl    = {https://dblp.org/rec/conf/nips/SongE19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@misc{urain2022se3diffusion,
  doi = {10.48550/ARXIV.2209.03855},
  url = {https://arxiv.org/abs/2209.03855},
  author = {Urain, Julen and Funk, Niklas and Peters, Jan and Chalvatzaki, Georgia},
  keywords = {Robotics (cs.RO), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {SE(3)-DiffusionFields: Learning smooth cost functions for joint grasp and motion optimization through diffusion},
  publisher = {arXiv},
  year = {2022},
  copyright = {Creative Commons Attribution 4.0 International}
}


@misc{openai2019rubik,
  doi = {10.48550/ARXIV.1910.07113},
  
  url = {https://arxiv.org/abs/1910.07113},
  
  author = {{OpenAI} and Akkaya, Ilge and Andrychowicz, Marcin and Chociej, Maciek and Litwin, Mateusz and McGrew, Bob and Petron, Arthur and Paino, Alex and Plappert, Matthias and Powell, Glenn and Ribas, Raphael and Schneider, Jonas and Tezak, Nikolas and Tworek, Jerry and Welinder, Peter and Weng, Lilian and Yuan, Qiming and Zaremba, Wojciech and Zhang, Lei},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), Computer Vision and Pattern Recognition (cs.CV), Robotics (cs.RO), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Solving Rubik's Cube with a Robot Hand},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{funk2022rrc,
  author =		 "Funk, N. and  Schaff, C. and  Madan, R. and  Yoneda, T. and  Urain, J. and  Watson, J. and  Gordon, E. and  Widmaier, F and  Bauer, S. and  Srinivasa, S. and  Bhattacharjee, T. and  Walter, M. and  Peters, J.",
  year =		 "2022",
  title =		 "Benchmarking Structured Policies and Policy Optimization for Real-World Dexterous Object Manipulation",
  booktitle =		 "IEEE Robotics and Automation Letters",
  URL =			 "https://www.ias.informatik.tu-darmstadt.de/uploads/Team/NiklasFunk/RRC_v1.pdf",
  number =		 "1",
  pages =		 "478-485",
}


@misc{rudin2021learningtowalk,
  doi = {10.48550/ARXIV.2109.11978},
  
  url = {https://arxiv.org/abs/2109.11978},
  
  author = {Rudin, Nikita and Hoeller, David and Reist, Philipp and Hutter, Marco},
  
  keywords = {Robotics (cs.RO), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Learning to Walk in Minutes Using Massively Parallel Deep Reinforcement Learning},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{narang2022factory,
  doi = {10.48550/ARXIV.2205.03532},
  
  url = {https://arxiv.org/abs/2205.03532},
  
  author = {Narang, Yashraj and Storey, Kier and Akinola, Iretiayo and Macklin, Miles and Reist, Philipp and Wawrzyniak, Lukasz and Guo, Yunrong and Moravanszky, Adam and State, Gavriel and Lu, Michelle and Handa, Ankur and Fox, Dieter},
  
  keywords = {Robotics (cs.RO), Graphics (cs.GR), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Factory: Fast Contact for Robotic Assembly},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{kumar2021rma,
  doi = {10.48550/ARXIV.2107.04034},
  
  url = {https://arxiv.org/abs/2107.04034},
  
  author = {Kumar, Ashish and Fu, Zipeng and Pathak, Deepak and Malik, Jitendra},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), Computer Vision and Pattern Recognition (cs.CV), Robotics (cs.RO), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {RMA: Rapid Motor Adaptation for Legged Robots},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{Lavalle98rapidly-exploringrandom,
    author = {Steven M. Lavalle},
    title = {Rapidly-Exploring Random Trees: A New Tool for Path Planning},
    year = {1998}
}

@INPROCEEDINGS{kuffner2000rrtstar,  
author={Kuffner, J.J. and LaValle, S.M.},  booktitle={Proceedings 2000 ICRA. Millennium Conference. IEEE International Conference on Robotics and Automation. Symposia Proceedings (Cat. No.00CH37065)},   title={RRT-connect: An efficient approach to single-query path planning},   year={2000},  volume={2},  number={},  pages={995-1001 vol.2},  doi={10.1109/ROBOT.2000.844730}}


@article{dam2022mcpp,
  author =		 "Dam, T. and  Chalvatzaki, G. and  Peters, J. and  Pajarinen J.",
  year =		 "2022",
  title =		 "Monte-Carlo Robot Path Planning",
  booktitle =		 "IEEE Robotics and Automation Letters, and 2022 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)",
  key =			 "planning under uncertainty, motion and path planning, planning, scheduling and coordination",
  URL =			 "https://www.ias.informatik.tu-darmstadt.de/uploads/Team/TuanDam/Monte_Carlo_Robot_Path_Planning_R_AL.pdf",
}


@inproceedings{Kalakrishnan_RAIIC_2011_stomp,
  title = {STOMP: Stochastic trajectory optimization for motion planning},
  author = {Kalakrishnan, M. and Chitta, S. and Theodorou, E. and Pastor, P. and Schaal, S.},
  booktitle = {IEEE International Conference on Robotics and Automation (ICRA)},
  address = {Shanghai, China, May 9-13},
  year = {2011},
  note = {clmc},
  doi = {},
  url = {http://www-clmc.usc.edu/publications/K/kalakrishnan-ICRA2011.pdf}
}



@inproceedings{urain_2022_learning_implicit_priors,
  author =		 "Urain, J. and  Le, A.T. and  Lambert, A. and  Chalvatzaki, G. and  Boots, B. and  Peters, J.",
  year =		 "2022",
  title =		 "Learning Implicit Priors for Motion Optimization",
  booktitle =		 "IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)",
  key =			 "motion planning, energy-based models",
  URL =			 "https://www.ias.informatik.tu-darmstadt.de/uploads/Team/AnThaiLe/iros2022_ebmtrajopt.pdf",
}


@InProceedings{Park_2019_CVPR_deepsdf,
author = {Park, Jeong Joon and Florence, Peter and Straub, Julian and Newcombe, Richard and Lovegrove, Steven},
title = {DeepSDF: Learning Continuous Signed Distance Functions for Shape Representation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}


@inproceedings{curless1996sdf,
author = {Curless, Brian and Levoy, Marc},
title = {A Volumetric Method for Building Complex Models from Range Images},
year = {1996},
isbn = {0897917464},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/237170.237269},
doi = {10.1145/237170.237269},
booktitle = {Proceedings of the 23rd Annual Conference on Computer Graphics and Interactive Techniques},
pages = {303–312},
numpages = {10},
keywords = {three-dimensional shape recovery, surface fitting, isosurface extraction, range image integration},
series = {SIGGRAPH '96}
}



@INPROCEEDINGS{ratliff2009chomp,  author={Ratliff, Nathan and Zucker, Matt and Bagnell, J. Andrew and Srinivasa, Siddhartha},  booktitle={2009 IEEE International Conference on Robotics and Automation},   title={CHOMP: Gradient optimization techniques for efficient motion planning},   year={2009},  volume={},  number={},  pages={489-494},  doi={10.1109/ROBOT.2009.5152817}}



@inproceedings{toussaint2009robusttrajopt,
author = {Toussaint, Marc},
title = {Robot Trajectory Optimization Using Approximate Inference},
year = {2009},
isbn = {9781605585161},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/1553374.1553508},
doi = {10.1145/1553374.1553508},
abstract = {The general stochastic optimal control (SOC) problem in robotics scenarios is often too complex to be solved exactly and in near real time. A classical approximate solution is to first compute an optimal (deterministic) trajectory and then solve a local linear-quadratic-gaussian (LQG) perturbation model to handle the system stochasticity. We present a new algorithm for this approach which improves upon previous algorithms like iLQG. We consider a probabilistic model for which the maximum likelihood (ML) trajectory coincides with the optimal trajectory and which, in the LQG case, reproduces the classical SOC solution. The algorithm then utilizes approximate inference methods (similar to expectation propagation) that efficiently generalize to non-LQG systems. We demonstrate the algorithm on a simulated 39-DoF humanoid robot.},
booktitle = {Proceedings of the 26th Annual International Conference on Machine Learning},
pages = {1049–1056},
numpages = {8},
location = {Montreal, Quebec, Canada},
series = {ICML '09}
}


@misc{levine2018rlcontrolasinference,
  doi = {10.48550/ARXIV.1805.00909},
  
  url = {https://arxiv.org/abs/1805.00909},
  
  author = {Levine, Sergey},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), Robotics (cs.RO), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Reinforcement Learning and Control as Probabilistic Inference: Tutorial and Review},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings{welling2011langevin,
author = {Welling, Max and Teh, Yee Whye},
title = {Bayesian Learning via Stochastic Gradient Langevin Dynamics},
year = {2011},
isbn = {9781450306195},
publisher = {Omnipress},
address = {Madison, WI, USA},
abstract = {In this paper we propose a new framework for learning from large scale datasets based on iterative learning from small mini-batches. By adding the right amount of noise to a standard stochastic gradient optimization algorithm we show that the iterates will converge to samples from the true posterior distribution as we anneal the stepsize. This seamless transition between optimization and Bayesian posterior sampling provides an inbuilt protection against overfitting. We also propose a practical method for Monte Carlo estimates of posterior statistics which monitors a "sampling threshold" and collects samples after it has been surpassed. We apply the method to three models: a mixture of Gaussians, logistic regression and ICA with natural gradients.},
booktitle = {Proceedings of the 28th International Conference on International Conference on Machine Learning},
pages = {681–688},
numpages = {8},
location = {Bellevue, Washington, USA},
series = {ICML'11}
}


@article{hyvarinen2005estimationscorematching,
  author  = {Aapo Hyv{{\"a}}rinen},
  title   = {Estimation of Non-Normalized Statistical Models by Score Matching},
  journal = {Journal of Machine Learning Research},
  year    = {2005},
  volume  = {6},
  number  = {24},
  pages   = {695--709},
  url     = {http://jmlr.org/papers/v6/hyvarinen05a.html}
}

@ARTICLE{vincent2011scorematching,  author={Vincent, Pascal},  journal={Neural Computation},   title={A Connection Between Score Matching and Denoising Autoencoders},   year={2011},  volume={23},  number={7},  pages={1661-1674},  doi={10.1162/NECO_a_00142}}


@misc{wang2022diffusionrl,
  doi = {10.48550/ARXIV.2208.06193},
  
  url = {https://arxiv.org/abs/2208.06193},
  
  author = {Wang, Zhendong and Hunt, Jonathan J and Zhou, Mingyuan},
  
  keywords = {Machine Learning (cs.LG), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Diffusion Policies as an Expressive Policy Class for Offline Reinforcement Learning},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}




@InProceedings{pascanu2013difficulttrainrnn,
  title = 	 {On the difficulty of training recurrent neural networks},
  author = 	 {Pascanu, Razvan and Mikolov, Tomas and Bengio, Yoshua},
  booktitle = 	 {Proceedings of the 30th International Conference on Machine Learning},
  pages = 	 {1310--1318},
  year = 	 {2013},
  editor = 	 {Dasgupta, Sanjoy and McAllester, David},
  volume = 	 {28},
  number =       {3},
  series = 	 {Proceedings of Machine Learning Research},
  address = 	 {Atlanta, Georgia, USA},
  month = 	 {17--19 Jun},
  publisher =    {PMLR},
  pdf = 	 {http://proceedings.mlr.press/v28/pascanu13.pdf},
  url = 	 {https://proceedings.mlr.press/v28/pascanu13.html},
  abstract = 	 {There are two widely known issues with properly training recurrent neural networks, the vanishing and the exploding gradient problems detailed in Bengio et al. (1994). In this paper we attempt to improve the understanding of the underlying issues by exploring these problems from an analytical, a geometric and a dynamical systems perspective. Our analysis is used to justify a simple yet effective solution. We propose a gradient norm clipping strategy to deal with exploding gradients and a soft constraint for the vanishing gradients problem. We validate empirically our hypothesis and proposed solutions in the experimental section.  }
}



@article{power2022variationalmpcnf,
place = {Country unknown/Code not available}, title = {Variational Inference MPC using Normalizing Flows and Out-of-Distribution Projection}, url = {https://par.nsf.gov/biblio/10348466}, DOI = {10.15607/RSS.2022.XVIII.027}, abstractNote = {}, journal = {Robotics: Science and Systems 2022.}, author = {Power, Thomas and Berenson, Dmitry}, year=2022}


@misc{ichter2017learningsamplingdist,
  doi = {10.48550/ARXIV.1709.05448},
  
  url = {https://arxiv.org/abs/1709.05448},
  
  author = {Ichter, Brian and Harrison, James and Pavone, Marco},
  
  keywords = {Robotics (cs.RO), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Learning Sampling Distributions for Robot Motion Planning},
  
  publisher = {arXiv},
  
  year = {2017},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@inproceedings{qureshi2018deepsmp,
  author    = {Ahmed Hussain Qureshi and
               Michael C. Yip},
  title     = {Deeply Informed Neural Sampling for Robot Motion Planning},
  booktitle = {2018 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2018, Madrid, Spain, October 1-5, 2018},
  pages     = {6582--6588},
  publisher = {{IEEE}},
  year      = {2018},
  url       = {https://doi.org/10.1109/IROS.2018.8593772},
  doi       = {10.1109/IROS.2018.8593772},
  timestamp = {Wed, 31 Mar 2021 09:15:02 +0200},
  biburl    = {https://dblp.org/rec/conf/iros/QureshiY18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Qureshi2018motionplanningnet,
  author    = {Ahmed Hussain Qureshi and
               Anthony Simeonov and
               Mayur J. Bency and
               Michael C. Yip},
  title     = {Motion Planning Networks},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019,
               Montreal, QC, Canada, May 20-24, 2019},
  pages     = {2118--2124},
  publisher = {{IEEE}},
  year      = {2019},
  doi       = {10.1109/ICRA.2019.8793889},
  timestamp = {Wed, 31 Mar 2021 09:15:03 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/QureshiSBY19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{Qureshi2020neuralmotionplanning,
  author    = {Ahmed Hussain Qureshi and
               Jiangeng Dong and
               Austin Choe and
               Michael C. Yip},
  title     = {Neural Manipulation Planning on Constraint Manifolds},
  journal   = {{IEEE} Robotics Autom. Lett.},
  volume    = {5},
  number    = {4},
  pages     = {6089--6096},
  year      = {2020},
  url       = {https://doi.org/10.1109/LRA.2020.3010220},
  doi       = {10.1109/LRA.2020.3010220},
  timestamp = {Wed, 31 Mar 2021 09:14:59 +0200},
  biburl    = {https://dblp.org/rec/journals/ral/QureshiDCY20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@ARTICLE{wang2020neuralrrt,
author={Wang, Jiankun and Chi, Wenzheng and Li, Chenming and Wang, Chaoqun and Meng, Max Q.-H.},  journal={IEEE Transactions on Automation Science and Engineering},   title={Neural RRT*: Learning-Based Optimal Path Planning},   year={2020},  volume={17},  number={4},  pages={1748-1758},  doi={10.1109/TASE.2020.2976560}}



@inproceedings{goodfellow2014gan,
 author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {Z. Ghahramani and M. Welling and C. Cortes and N. Lawrence and K.Q. Weinberger},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Generative Adversarial Nets},
 url = {https://proceedings.neurips.cc/paper/2014/file/5ca3e9b122f61f8f06494c97b1afccf3-Paper.pdf},
 volume = {27},
 year = {2014}
}



@inproceedings{kingma2013vae,
  author    = {Diederik P. Kingma and
               Max Welling},
  editor    = {Yoshua Bengio and
               Yann LeCun},
  title     = {Auto-Encoding Variational Bayes},
  booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
               Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
  year      = {2014},
  url       = {http://arxiv.org/abs/1312.6114},
  timestamp = {Thu, 04 Apr 2019 13:20:07 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/KingmaW13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}




@inproceedings{rezende2015nf,
  author    = {Danilo Jimenez Rezende and
               Shakir Mohamed},
  editor    = {Francis R. Bach and
               David M. Blei},
  title     = {Variational Inference with Normalizing Flows},
  booktitle = {Proceedings of the 32nd International Conference on Machine Learning,
               {ICML} 2015, Lille, France, 6-11 July 2015},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {37},
  pages     = {1530--1538},
  publisher = {JMLR.org},
  year      = {2015},
  url       = {http://proceedings.mlr.press/v37/rezende15.html},
  timestamp = {Wed, 29 May 2019 08:41:45 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/RezendeM15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}





@inproceedings{ho2020denoisingdiffusion,
author = {Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
title = {Denoising Diffusion Probabilistic Models},
year = {2020},
isbn = {9781713829546},
publisher = {Curran Associates Inc.},
address = {Red Hook, NY, USA},
abstract = {We present high quality image synthesis results using diffusion probabilistic models, a class of latent variable models inspired by considerations from nonequilibrium thermodynamics. Our best results are obtained by training on a weighted variational bound designed according to a novel connection between diffusion probabilistic models and denoising score matching with Langevin dynamics, and our models naturally admit a progressive lossy decompression scheme that can be interpreted as a generalization of autoregressive decoding. On the unconditional CIFAR10 dataset, we obtain an Inception score of 9.46 and a state-of-the-art FID score of 3.17. On 256x256 LSUN, we obtain sample quality similar to ProgressiveGAN.},
booktitle = {Proceedings of the 34th International Conference on Neural Information Processing Systems},
articleno = {574},
numpages = {12},
location = {Vancouver, BC, Canada},
series = {NIPS'20}
}



@InProceedings{Kim_2022_CVPR,
    author    = {Kim, Gwanghyun and Kwon, Taesung and Ye, Jong Chul},
    title     = {DiffusionCLIP: Text-Guided Diffusion Models for Robust Image Manipulation},
    booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
    month     = {June},
    year      = {2022},
    pages     = {2426-2435}
}



@misc{ramesh2022dalle2,
  doi = {10.48550/ARXIV.2204.06125},
  
  url = {https://arxiv.org/abs/2204.06125},
  
  author = {Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Hierarchical Text-Conditional Image Generation with CLIP Latents},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}



@ARTICLE{Kavraki1996PRM,  author={Kavraki, L.E. and Svestka, P. and Latombe, J.-C. and Overmars, M.H.},  journal={IEEE Transactions on Robotics and Automation},   title={Probabilistic roadmaps for path planning in high-dimensional configuration spaces},   year={1996},  volume={12},  number={4},  pages={566-580},  doi={10.1109/70.508439}}



@misc{huang2022innermonologue,
  doi = {10.48550/ARXIV.2207.05608},
  
  url = {https://arxiv.org/abs/2207.05608},
  
  author = {Huang, Wenlong and Xia, Fei and Xiao, Ted and Chan, Harris and Liang, Jacky and Florence, Pete and Zeng, Andy and Tompson, Jonathan and Mordatch, Igor and Chebotar, Yevgen and Sermanet, Pierre and Brown, Noah and Jackson, Tomas and Luu, Linda and Levine, Sergey and Hausman, Karol and Ichter, Brian},
  
  keywords = {Robotics (cs.RO), Artificial Intelligence (cs.AI), Computation and Language (cs.CL), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Inner Monologue: Embodied Reasoning through Planning with Language Models},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@inproceedings{Simeonov2022neuraldescriptorfields,
  author    = {Anthony Simeonov and
               Yilun Du and
               Andrea Tagliasacchi and
               Joshua B. Tenenbaum and
               Alberto Rodriguez and
               Pulkit Agrawal and
               Vincent Sitzmann},
  title     = {Neural Descriptor Fields: SE(3)-Equivariant Object Representations
               for Manipulation},
  booktitle = {2022 International Conference on Robotics and Automation, {ICRA} 2022,
               Philadelphia, PA, USA, May 23-27, 2022},
  pages     = {6394--6400},
  publisher = {{IEEE}},
  year      = {2022},
  url       = {https://doi.org/10.1109/ICRA46639.2022.9812146},
  doi       = {10.1109/ICRA46639.2022.9812146},
  timestamp = {Wed, 20 Jul 2022 18:22:50 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/SimeonovDTT0AS22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}




@inproceedings{rana2017towardsrobustskill,
  author    = {Muhammad Asif Rana and
               Mustafa Mukadam and
               Seyed Reza Ahmadzadeh and
               Sonia Chernova and
               Byron Boots},
  title     = {Towards Robust Skill Generalization: Unifying Learning from Demonstration
               and Motion Planning},
  booktitle = {1st Annual Conference on Robot Learning, CoRL 2017, Mountain View,
               California, USA, November 13-15, 2017, Proceedings},
  series    = {Proceedings of Machine Learning Research},
  volume    = {78},
  pages     = {109--118},
  publisher = {{PMLR}},
  year      = {2017},
  url       = {http://proceedings.mlr.press/v78/rana17a.html},
  timestamp = {Wed, 03 Apr 2019 18:17:24 +0200},
  biburl    = {https://dblp.org/rec/conf/corl/RanaMACB17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@INPROCEEDINGS{koert2016debato,  author={Koert, Dorothea and Maeda, Guilherme and Lioutikov, Rudolf and Neumann, Gerhard and Peters, Jan},  booktitle={2016 IEEE-RAS 16th International Conference on Humanoid Robots (Humanoids)},   title={Demonstration based trajectory optimization for generalizable robot motions},   year={2016},  volume={},  number={},  pages={515-522},  doi={10.1109/HUMANOIDS.2016.7803324}}




@InProceedings{ortiz2022structureddeep,
  title = 	 {Structured deep generative models for sampling on constraint manifolds in sequential manipulation},
  author =       {Ortiz-Haro, Joaquim and Ha, Jung-Su and Driess, Danny and Toussaint, Marc},
  booktitle = 	 {Proceedings of the 5th Conference on Robot Learning},
  pages = 	 {213--223},
  year = 	 {2022},
  editor = 	 {Faust, Aleksandra and Hsu, David and Neumann, Gerhard},
  volume = 	 {164},
  series = 	 {Proceedings of Machine Learning Research},
  month = 	 {08--11 Nov},
  publisher =    {PMLR},
  pdf = 	 {https://proceedings.mlr.press/v164/ortiz-haro22a/ortiz-haro22a.pdf},
  url = 	 {https://proceedings.mlr.press/v164/ortiz-haro22a.html},
  abstract = 	 {Sampling efficiently on constraint manifolds is a core problem in robotics. We propose Deep Generative Constraint Sampling (DGCS), which combines a deep generative model for sampling close to a constraint manifold with nonlinear constrained optimization to project to the constraint manifold. The generative model is conditioned on the problem instance, taking a scene image as input, and it is trained with a dataset of solutions and a novel analytic constraint term. To further improve the precision and diversity of samples, we extend the approach to exploit a factorization of the constrained problem. We evaluate our approach in two problems of robotic sequential manipulation in cluttered environments. Experimental results demonstrate that our deep generative model produces diverse and precise samples and outperforms heuristic warmstart initialization. }
}



@inproceedings{Chamzas2021learningsampling,
  author    = {Constantinos Chamzas and
               Zachary K. Kingston and
               Carlos Quintero{-}Pe{\~{n}}a and
               Anshumali Shrivastava and
               Lydia E. Kavraki},
  title     = {Learning Sampling Distributions Using Local 3D Workspace Decompositions
               for Motion Planning in High Dimensions},
  booktitle = {{IEEE} International Conference on Robotics and Automation, {ICRA}
               2021, Xi'an, China, May 30 - June 5, 2021},
  pages     = {1283--1289},
  publisher = {{IEEE}},
  year      = {2021},
  url       = {https://doi.org/10.1109/ICRA48506.2021.9561104},
  doi       = {10.1109/ICRA48506.2021.9561104},
  timestamp = {Fri, 22 Oct 2021 19:57:12 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/ChamzasKQSK21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Cheng2020learningoptimalsampling,
  author    = {Richard Cheng and
               Krishna Shankar and
               Joel W. Burdick},
  title     = {Learning an Optimal Sampling Distribution for Efficient Motion Planning},
  booktitle = {{IEEE/RSJ} International Conference on Intelligent Robots and Systems,
               {IROS} 2020, Las Vegas, NV, USA, October 24, 2020 - January 24, 2021},
  pages     = {7485--7492},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/IROS45743.2020.9341245},
  doi       = {10.1109/IROS45743.2020.9341245},
  timestamp = {Tue, 16 Feb 2021 19:08:20 +0100},
  biburl    = {https://dblp.org/rec/conf/iros/ChengSB20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Kicki2021learningfromexperience,
  author    = {Piotr Kicki and
               Tomasz Gawron and
               Krzysztof Cwian and
               Mete Ozay and
               Piotr Skrzypczynski},
  title     = {Learning from experience for rapid generation of local car maneuvers},
  journal   = {Eng. Appl. Artif. Intell.},
  volume    = {105},
  pages     = {104399},
  year      = {2021},
  url       = {https://doi.org/10.1016/j.engappai.2021.104399},
  doi       = {10.1016/j.engappai.2021.104399},
  timestamp = {Tue, 05 Oct 2021 10:00:41 +0200},
  biburl    = {https://dblp.org/rec/journals/eaai/KickiGCOS21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Mukadam2018-gpmp-ijrr,
  author    = {Mustafa Mukadam and
               Jing Dong and
               Xinyan Yan and
               Frank Dellaert and
               Byron Boots},
  title     = {Continuous-time Gaussian process motion planning via probabilistic
               inference},
  journal   = {Int. J. Robotics Res.},
  volume    = {37},
  number    = {11},
  year      = {2018},
  url       = {https://doi.org/10.1177/0278364918790369},
  doi       = {10.1177/0278364918790369},
  timestamp = {Thu, 17 Sep 2020 12:02:45 +0200},
  biburl    = {https://dblp.org/rec/journals/ijrr/MukadamDYDB18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{Dong2016-gpmp-rss,
  Author = {Jing Dong and Mustafa Mukadam and Frank Dellaert and Byron Boots},
  Title = {Motion Planning as Probabilistic Inference using {G}aussian Processes and Factor Graphs},
  booktitle = {Proceedings of Robotics: Science and Systems (RSS)},
  year = {2016}
}

@inproceedings{dong2018sparse,
  title={Sparse {G}aussian Processes on Matrix {L}ie Groups: A Unified Framework for Optimizing Continuous-Time Trajectories},
  author={Dong, Jing and Mukadam, Mustafa and Boots, Byron and Dellaert, Frank},
  booktitle={2018 IEEE International Conference on Robotics and Automation (ICRA)},
  pages={6497--6504},
  year={2018},
  organization={IEEE}
}


@article{paraschos2018using,
  title={Using probabilistic movement primitives in robotics},
  author={Paraschos, Alexandros and Daniel, Christian and Peters, Jan and Neumann, Gerhard},
  journal={Autonomous Robots},
  volume={42},
  number={3},
  pages={529--551},
  year={2018},
  publisher={Springer}
}


@inproceedings{peters2010reps,
author = {Peters, Jan and M\"{u}lling, Katharina and Alt\"{u}n, Yasemin},
title = {Relative Entropy Policy Search},
year = {2010},
publisher = {AAAI Press},
abstract = {Policy search is a successful approach to reinforcement learning. However, policy improvements often result in the loss of information. Hence, it has been marred by premature convergence and implausible solutions. As first suggested in the context of covariant policy gradients (Bagnell and Schneider 2003), many of these problems may be addressed by constraining the information loss. In this paper, we continue this path of reasoning and suggest the Relative Entropy Policy Search (REPS) method. The resulting method differs significantly from previous policy gradient approaches and yields an exact update step. It works well on typical reinforcement learning benchmark problems.},
booktitle = {Proceedings of the Twenty-Fourth AAAI Conference on Artificial Intelligence},
pages = {1607–1612},
numpages = {6},
location = {Atlanta, Georgia},
series = {AAAI'10}
}



@inproceedings{Chamzas2019usinglocalexperiences,
  author    = {Constantinos Chamzas and
               Anshumali Shrivastava and
               Lydia E. Kavraki},
  title     = {Using Local Experiences for Global Motion Planning},
  booktitle = {International Conference on Robotics and Automation, {ICRA} 2019,
               Montreal, QC, Canada, May 20-24, 2019},
  pages     = {8606--8612},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/ICRA.2019.8794317},
  doi       = {10.1109/ICRA.2019.8794317},
  timestamp = {Sun, 25 Jul 2021 11:50:10 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/ChamzasSK19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@book{Lav2006planningalgorithms,
  author       = {S. M. LaValle},
  title        = {Planning Algorithms},
  publisher    = {Cambridge University Press},
  address      = {Cambridge, U.K.},
  year         = {2006}
}


@inproceedings{Schulman2013trajopt,
  author    = {John Schulman and
               Jonathan Ho and
               Alex X. Lee and
               Ibrahim Awwal and
               Henry Bradlow and
               Pieter Abbeel},
  editor    = {Paul Newman and
               Dieter Fox and
               David Hsu},
  title     = {Finding Locally Optimal, Collision-Free Trajectories with Sequential
               Convex Optimization},
  booktitle = {Robotics: Science and Systems IX, Technische Universit{\"{a}}t
               Berlin, Berlin, Germany, June 24 - June 28, 2013},
  year      = {2013},
  url       = {http://www.roboticsproceedings.org/rss09/p31.html},
  doi       = {10.15607/RSS.2013.IX.031},
  timestamp = {Fri, 29 Jan 2021 22:08:09 +0100},
  biburl    = {https://dblp.org/rec/conf/rss/SchulmanHLABA13.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@ARTICLE{petrovic2022mixturegp,  author={Petrović, Luka and Marković, Ivan and Petrović, Ivan},  journal={IEEE Transactions on Systems, Man, and Cybernetics: Systems},   title={Mixtures of Gaussian Processes for Robot Motion Planning Using Stochastic Trajectory Optimization},   year={2022},  volume={},  number={},  pages={1-13},  doi={10.1109/TSMC.2022.3155378}}



@article{florence2021implicit,
    title={Implicit Behavioral Cloning},
    author={Florence, Pete and Lynch, Corey and Zeng, Andy and Ramirez, Oscar and Wahid, Ayzaan and Downs, Laura and Wong, Adrian and Lee, Johnny and Mordatch, Igor and Tompson, Jonathan},
    journal={Conference on Robot Learning (CoRL)},
    year={2021}
}

@article{theodorou2010pathintegral,
  author  = {Evangelos Theodorou and Jonas Buchli and Stefan Schaal},
  title   = {A Generalized Path Integral Control Approach to Reinforcement Learning},
  journal = {Journal of Machine Learning Research},
  year    = {2010},
  volume  = {11},
  number  = {104},
  pages   = {3137--3181},
  url     = {http://jmlr.org/papers/v11/theodorou10a.html}
}


@inproceedings{watson2019i2c,
  author    = {Joe Watson and
               Hany Abdulsamad and
               Jan Peters},
  editor    = {Leslie Pack Kaelbling and
               Danica Kragic and
               Komei Sugiura},
  title     = {Stochastic Optimal Control as Approximate Input Inference},
  booktitle = {3rd Annual Conference on Robot Learning, CoRL 2019, Osaka, Japan,
               October 30 - November 1, 2019, Proceedings},
  series    = {Proceedings of Machine Learning Research},
  volume    = {100},
  pages     = {697--716},
  publisher = {{PMLR}},
  year      = {2019},
  url       = {http://proceedings.mlr.press/v100/watson20a.html},
  timestamp = {Mon, 25 May 2020 15:01:26 +0200},
  biburl    = {https://dblp.org/rec/conf/corl/WatsonA019.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{watson2021acc,
  author    = {Joe Watson and
               Jan Peters},
  title     = {Advancing Trajectory Optimization with Approximate Inference: Exploration,
               Covariance Control and Adaptive Risk},
  booktitle = {2021 American Control Conference, {ACC} 2021, New Orleans, LA, USA,
               May 25-28, 2021},
  pages     = {1231--1236},
  publisher = {{IEEE}},
  year      = {2021},
  url       = {https://doi.org/10.23919/ACC50511.2021.9482657},
  doi       = {10.23919/ACC50511.2021.9482657},
  timestamp = {Fri, 30 Jul 2021 11:11:53 +0200},
  biburl    = {https://dblp.org/rec/conf/amcc/Watson021.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Takayuki2018imitationlearning,
  author    = {Takayuki Osa and
               Joni Pajarinen and
               Gerhard Neumann and
               J. Andrew Bagnell and
               Pieter Abbeel and
               Jan Peters},
  title     = {An Algorithmic Perspective on Imitation Learning},
  journal   = {Found. Trends Robotics},
  volume    = {7},
  number    = {1-2},
  pages     = {1--179},
  year      = {2018},
  url       = {https://doi.org/10.1561/2300000053},
  doi       = {10.1561/2300000053},
  timestamp = {Thu, 10 Sep 2020 13:17:41 +0200},
  biburl    = {https://dblp.org/rec/journals/ftrob/OsaPNBA018.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{zhang2018learningimplicit,
  author    = {Clark Zhang and
               Jinwook Huh and
               Daniel D. Lee},
  title     = {Learning Implicit Sampling Distributions for Motion Planning},
  booktitle = {2018 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2018, Madrid, Spain, October 1-5, 2018},
  pages     = {3654--3661},
  publisher = {{IEEE}},
  year      = {2018},
  url       = {https://doi.org/10.1109/IROS.2018.8594028},
  doi       = {10.1109/IROS.2018.8594028},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iros/ZhangHL18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{bency2019neuralpathplanning,
  author    = {Mayur J. Bency and
               Ahmed Hussain Qureshi and
               Michael C. Yip},
  title     = {Neural Path Planning: Fixed Time, Near-Optimal Path Generation via
               Oracle Imitation},
  booktitle = {2019 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, {IROS} 2019, Macau, SAR, China, November 3-8, 2019},
  pages     = {3965--3972},
  publisher = {{IEEE}},
  year      = {2019},
  url       = {https://doi.org/10.1109/IROS40897.2019.8968089},
  doi       = {10.1109/IROS40897.2019.8968089},
  timestamp = {Wed, 31 Mar 2021 09:15:02 +0200},
  biburl    = {https://dblp.org/rec/conf/iros/BencyQY19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@book{latombe1991robotmotionplanning,
author = {Latombe, Jean-Claude},
title = {Robot Motion Planning},
year = {1991},
isbn = {0792391292},
publisher = {Kluwer Academic Publishers},
address = {USA}
}


@inproceedings{jurgenson2019harnessingrlnmp,
  author    = {Tom Jurgenson and
               Aviv Tamar},
  editor    = {Antonio Bicchi and
               Hadas Kress{-}Gazit and
               Seth Hutchinson},
  title     = {Harnessing Reinforcement Learning for Neural Motion Planning},
  booktitle = {Robotics: Science and Systems XV, University of Freiburg, Freiburg
               im Breisgau, Germany, June 22-26, 2019},
  year      = {2019},
  url       = {https://doi.org/10.15607/RSS.2019.XV.026},
  doi       = {10.15607/RSS.2019.XV.026},
  timestamp = {Thu, 01 Apr 2021 15:25:13 +0200},
  biburl    = {https://dblp.org/rec/conf/rss/JurgensonT19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{strudel2020learningobstaclerepresentationsfornmp,
  author    = {Robin Strudel and
               Ricardo Garcia Pinel and
               Justin Carpentier and
               Jean{-}Paul Laumond and
               Ivan Laptev and
               Cordelia Schmid},
  editor    = {Jens Kober and
               Fabio Ramos and
               Claire J. Tomlin},
  title     = {Learning Obstacle Representations for Neural Motion Planning},
  booktitle = {4th Conference on Robot Learning, CoRL 2020, 16-18 November 2020,
               Virtual Event / Cambridge, MA, {USA}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {155},
  pages     = {355--364},
  publisher = {{PMLR}},
  year      = {2020},
  url       = {https://proceedings.mlr.press/v155/strudel21a.html},
  timestamp = {Mon, 25 Oct 2021 15:03:56 +0200},
  biburl    = {https://dblp.org/rec/conf/corl/StrudelPCLLS20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{qi2017pointnet,
  author    = {Charles Ruizhongtai Qi and
               Hao Su and
               Kaichun Mo and
               Leonidas J. Guibas},
  title     = {PointNet: Deep Learning on Point Sets for 3D Classification and Segmentation},
  booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
               {CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
  pages     = {77--85},
  publisher = {{IEEE} Computer Society},
  year      = {2017},
  url       = {https://doi.org/10.1109/CVPR.2017.16},
  doi       = {10.1109/CVPR.2017.16},
  timestamp = {Wed, 11 Nov 2020 08:48:18 +0100},
  biburl    = {https://dblp.org/rec/conf/cvpr/QiSMG17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@misc{chen2022offrlhighfidelity,
  doi = {10.48550/ARXIV.2209.14548},
  
  url = {https://arxiv.org/abs/2209.14548},
  
  author = {Chen, Huayu and Lu, Cheng and Ying, Chengyang and Su, Hang and Zhu, Jun},
  
  keywords = {Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Offline Reinforcement Learning via High-Fidelity Generative Behavior Modeling},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@misc{zhang2022motiondiffuse,
  doi = {10.48550/ARXIV.2208.15001},
  
  url = {https://arxiv.org/abs/2208.15001},
  
  author = {Zhang, Mingyuan and Cai, Zhongang and Pan, Liang and Hong, Fangzhou and Guo, Xinying and Yang, Lei and Liu, Ziwei},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {MotionDiffuse: Text-Driven Human Motion Generation with Diffusion Model},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{tevet2022humanmotiondiffusion,
  doi = {10.48550/ARXIV.2209.14916},
  
  url = {https://arxiv.org/abs/2209.14916},
  
  author = {Tevet, Guy and Raab, Sigal and Gordon, Brian and Shafir, Yonatan and Cohen-Or, Daniel and Bermano, Amit H.},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Graphics (cs.GR), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Human Motion Diffusion Model},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Share Alike 4.0 International}
}



@misc{findlay2022ddpmwalking,
  doi = {10.48550/ARXIV.2209.14828},
  
  url = {https://arxiv.org/abs/2209.14828},
  
  author = {Findlay, Edmund J. C. and Zhang, Haozheng and Chang, Ziyi and Shum, Hubert P. H.},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Graphics (cs.GR), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Denoising Diffusion Probabilistic Models for Styled Walking Synthesis},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings{deng2021vnn,
  author    = {Congyue Deng and
               Or Litany and
               Yueqi Duan and
               Adrien Poulenard and
               Andrea Tagliasacchi and
               Leonidas J. Guibas},
  title     = {Vector Neurons: {A} General Framework for SO(3)-Equivariant Networks},
  booktitle = {2021 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
               2021, Montreal, QC, Canada, October 10-17, 2021},
  pages     = {12180--12189},
  publisher = {{IEEE}},
  year      = {2021},
  url       = {https://doi.org/10.1109/ICCV48922.2021.01198},
  doi       = {10.1109/ICCV48922.2021.01198},
  timestamp = {Fri, 11 Mar 2022 10:01:59 +0100},
  biburl    = {https://dblp.org/rec/conf/iccv/DengLDPTG21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{wang2019dgcnn,
  author    = {Yue Wang and
               Yongbin Sun and
               Ziwei Liu and
               Sanjay E. Sarma and
               Michael M. Bronstein and
               Justin M. Solomon},
  title     = {Dynamic Graph {CNN} for Learning on Point Clouds},
  journal   = {{ACM} Trans. Graph.},
  volume    = {38},
  number    = {5},
  pages     = {146:1--146:12},
  year      = {2019},
  url       = {https://doi.org/10.1145/3326362},
  doi       = {10.1145/3326362},
  timestamp = {Tue, 02 Aug 2022 14:54:57 +0200},
  biburl    = {https://dblp.org/rec/journals/tog/WangSLSBS19.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{qureshi2021mpn-tro,
  author    = {Ahmed Hussain Qureshi and
               Yinglong Miao and
               Anthony Simeonov and
               Michael C. Yip},
  title     = {Motion Planning Networks: Bridging the Gap Between Learning-Based
               and Classical Motion Planners},
  journal   = {{IEEE} Trans. Robotics},
  volume    = {37},
  number    = {1},
  pages     = {48--66},
  year      = {2021},
  url       = {https://doi.org/10.1109/TRO.2020.3006716},
  doi       = {10.1109/TRO.2020.3006716},
  timestamp = {Wed, 31 Mar 2021 09:14:59 +0200},
  biburl    = {https://dblp.org/rec/journals/trob/QureshiMSY21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{Ichnowski2020dj-gomp,
  author    = {Jeffrey Ichnowski and
               Yahav Avigal and
               Vishal Satish and
               Ken Goldberg},
  title     = {Deep learning can accelerate grasp-optimized motion planning},
  journal   = {Sci. Robotics},
  volume    = {5},
  number    = {48},
  pages     = {7710},
  year      = {2020},
  url       = {https://doi.org/10.1126/scirobotics.abd7710},
  doi       = {10.1126/scirobotics.abd7710},
  timestamp = {Wed, 16 Mar 2022 23:49:49 +0100},
  biburl    = {https://dblp.org/rec/journals/scirobotics/AvigalSG20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{liang2022codeaspolicies,
  author    = {Jacky Liang and
               Wenlong Huang and
               Fei Xia and
               Peng Xu and
               Karol Hausman and
               Brian Ichter and
               Pete Florence and
               Andy Zeng},
  title     = {Code as Policies: Language Model Programs for Embodied Control},
  journal   = {CoRR},
  volume    = {abs/2209.07753},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2209.07753},
  doi       = {10.48550/arXiv.2209.07753},
  eprinttype = {arXiv},
  eprint    = {2209.07753},
  timestamp = {Tue, 27 Sep 2022 16:29:43 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2209-07753.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{shridhar2022perceiveractor,
  author    = {Mohit Shridhar and
               Lucas Manuelli and
               Dieter Fox},
  title     = {Perceiver-Actor: {A} Multi-Task Transformer for Robotic Manipulation},
  journal   = {CoRR},
  volume    = {abs/2209.05451},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2209.05451},
  doi       = {10.48550/arXiv.2209.05451},
  eprinttype = {arXiv},
  eprint    = {2209.05451},
  timestamp = {Tue, 27 Sep 2022 16:29:43 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2209-05451.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{ahn2022saycan,
  author    = {Michael Ahn and
               Anthony Brohan and
               Noah Brown and
               Yevgen Chebotar and
               Omar Cortes and
               Byron David and
               Chelsea Finn and
               Keerthana Gopalakrishnan and
               Karol Hausman and
               Alexander Herzog and
               Daniel Ho and
               Jasmine Hsu and
               Julian Ibarz and
               Brian Ichter and
               Alex Irpan and
               Eric Jang and
               Rosario Jauregui Ruano and
               Kyle Jeffrey and
               Sally Jesmonth and
               Nikhil J. Joshi and
               Ryan Julian and
               Dmitry Kalashnikov and
               Yuheng Kuang and
               Kuang{-}Huei Lee and
               Sergey Levine and
               Yao Lu and
               Linda Luu and
               Carolina Parada and
               Peter Pastor and
               Jornell Quiambao and
               Kanishka Rao and
               Jarek Rettinghouse and
               Diego Reyes and
               Pierre Sermanet and
               Nicolas Sievers and
               Clayton Tan and
               Alexander Toshev and
               Vincent Vanhoucke and
               Fei Xia and
               Ted Xiao and
               Peng Xu and
               Sichun Xu and
               Mengyuan Yan},
  title     = {Do As {I} Can, Not As {I} Say: Grounding Language in Robotic Affordances},
  journal   = {CoRR},
  volume    = {abs/2204.01691},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2204.01691},
  doi       = {10.48550/arXiv.2204.01691},
  eprinttype = {arXiv},
  eprint    = {2204.01691},
  timestamp = {Tue, 16 Aug 2022 23:07:05 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2204-01691.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@ARTICLE{hart1968astar,
  author={Hart, Peter E. and Nilsson, Nils J. and Raphael, Bertram},
  journal={IEEE Transactions on Systems Science and Cybernetics}, 
  title={A Formal Basis for the Heuristic Determination of Minimum Cost Paths}, 
  year={1968},
  volume={4},
  number={2},
  pages={100-107},
  doi={10.1109/TSSC.1968.300136}}



@article{lemmon1991-2dofrobot,
    author = {Lemmon, Michael},
    title = "{2-Degree-of-freedom Robot Path Planning using Cooperative Neural Fields}",
    journal = {Neural Computation},
    volume = {3},
    number = {3},
    pages = {350-362},
    year = {1991},
    month = {09},
    abstract = "{This paper proposes a neural network solution to path planning by two degree-of-freedom (DOF) robots. The proposed network is a two-dimensional sheet of neurons forming a distributed representation of the robot's workspace. Lateral interconnections between neurons are “cooperative,” so that the field exhibits oscillatory behavior. This paper shows how that oscillatory behavior can be used to solve the path-planning problem. The results reported show that the proposed neural network finds the variational solution of Bellman's dynamic programming equation.}",
    issn = {0899-7667},
    doi = {10.1162/neco.1991.3.3.350},
    url = {https://doi.org/10.1162/neco.1991.3.3.350},
    eprint = {https://direct.mit.edu/neco/article-pdf/3/3/350/812159/neco.1991.3.3.350.pdf},
}

@inproceedings{lemmon1991-oscillatory,
 author = {Lemmon, Michael},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {J. Moody and S. Hanson and R.P. Lippmann},
 pages = {},
 publisher = {Morgan-Kaufmann},
 title = {Oscillatory Neural Fields for Globally Optimal Path Planning},
 url = {https://proceedings.neurips.cc/paper/1991/file/c9892a989183de32e976c6f04e700201-Paper.pdf},
 volume = {4},
 year = {1991}
}


@inproceedings{bhardwaj2021storm,
  author    = {Mohak Bhardwaj and
               Balakumar Sundaralingam and
               Arsalan Mousavian and
               Nathan D. Ratliff and
               Dieter Fox and
               Fabio Ramos and
               Byron Boots},
  editor    = {Aleksandra Faust and
               David Hsu and
               Gerhard Neumann},
  title     = {{STORM:} An Integrated Framework for Fast Joint-Space Model-Predictive
               Control for Reactive Manipulation},
  booktitle = {Conference on Robot Learning, 8-11 November 2021, London, {UK}},
  series    = {Proceedings of Machine Learning Research},
  volume    = {164},
  pages     = {750--759},
  publisher = {{PMLR}},
  year      = {2021},
  url       = {https://proceedings.mlr.press/v164/bhardwaj22a.html},
  timestamp = {Wed, 19 Jan 2022 17:10:33 +0100},
  biburl    = {https://dblp.org/rec/conf/corl/BhardwajSMRFRB21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{zeng2022socraticmodels,
  author    = {Andy Zeng and
               Adrian Wong and
               Stefan Welker and
               Krzysztof Choromanski and
               Federico Tombari and
               Aveek Purohit and
               Michael S. Ryoo and
               Vikas Sindhwani and
               Johnny Lee and
               Vincent Vanhoucke and
               Pete Florence},
  title     = {Socratic Models: Composing Zero-Shot Multimodal Reasoning with Language},
  journal   = {CoRR},
  volume    = {abs/2204.00598},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2204.00598},
  doi       = {10.48550/arXiv.2204.00598},
  eprinttype = {arXiv},
  eprint    = {2204.00598},
  timestamp = {Wed, 06 Apr 2022 14:29:31 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2204-00598.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{lambert2022svprm,
  author    = {Alexander Lambert and
               Brian Hou and
               Rosario Scalise and
               Siddhartha S. Srinivasa and
               Byron Boots},
  title     = {Stein Variational Probabilistic Roadmaps},
  booktitle = {2022 International Conference on Robotics and Automation, {ICRA} 2022,
               Philadelphia, PA, USA, May 23-27, 2022},
  pages     = {11094--11101},
  publisher = {{IEEE}},
  year      = {2022},
  url       = {https://doi.org/10.1109/ICRA46639.2022.9811656},
  doi       = {10.1109/ICRA46639.2022.9811656},
  timestamp = {Thu, 21 Jul 2022 10:38:29 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/LambertHSSB22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{yu2022gvi,
  author    = {Hongzhe Yu and
               Yongxin Chen},
  title     = {A Gaussian variational inference approach to motion planning},
  journal   = {CoRR},
  volume    = {abs/2209.05655},
  year      = {2022},
  url       = {https://doi.org/10.48550/arXiv.2209.05655},
  doi       = {10.48550/arXiv.2209.05655},
  eprinttype = {arXiv},
  eprint    = {2209.05655},
  timestamp = {Tue, 27 Sep 2022 16:29:43 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2209-05655.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@article{lambert2021entropyregmp-svgd,
  author    = {Alexander Lambert and
               Byron Boots},
  title     = {Entropy Regularized Motion Planning via Stein Variational Inference},
  journal   = {CoRR},
  volume    = {abs/2107.05146},
  year      = {2021},
  url       = {https://arxiv.org/abs/2107.05146},
  eprinttype = {arXiv},
  eprint    = {2107.05146},
  timestamp = {Tue, 20 Jul 2021 15:08:33 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2107-05146.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@inproceedings{Jaderberg2017-rl-unsupervised,
  author    = {Max Jaderberg and
               Volodymyr Mnih and
               Wojciech Marian Czarnecki and
               Tom Schaul and
               Joel Z. Leibo and
               David Silver and
               Koray Kavukcuoglu},
  title     = {Reinforcement Learning with Unsupervised Auxiliary Tasks},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
               Toulon, France, April 24-26, 2017, Conference Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2017},
  url       = {https://openreview.net/forum?id=SJ6yPD5xg},
  timestamp = {Thu, 14 Oct 2021 10:00:37 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/JaderbergMCSLSK17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Schwarzer2021-spr,
  author    = {Max Schwarzer and
               Ankesh Anand and
               Rishab Goel and
               R. Devon Hjelm and
               Aaron C. Courville and
               Philip Bachman},
  title     = {Data-Efficient Reinforcement Learning with Self-Predictive Representations},
  booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
               Virtual Event, Austria, May 3-7, 2021},
  publisher = {OpenReview.net},
  year      = {2021},
  url       = {https://openreview.net/forum?id=uCQfPZwRaUu},
  timestamp = {Wed, 23 Jun 2021 17:36:39 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/SchwarzerAGHCB21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Andreas2018-learninglatentlanguage,
  author    = {Jacob Andreas and
               Dan Klein and
               Sergey Levine},
  editor    = {Marilyn A. Walker and
               Heng Ji and
               Amanda Stent},
  title     = {Learning with Latent Language},
  booktitle = {Proceedings of the 2018 Conference of the North American Chapter of
               the Association for Computational Linguistics: Human Language Technologies,
               {NAACL-HLT} 2018, New Orleans, Louisiana, USA, June 1-6, 2018, Volume
               1 (Long Papers)},
  pages     = {2166--2179},
  publisher = {Association for Computational Linguistics},
  year      = {2018},
  url       = {https://doi.org/10.18653/v1/n18-1197},
  doi       = {10.18653/v1/n18-1197},
  timestamp = {Fri, 06 Aug 2021 00:41:32 +0200},
  biburl    = {https://dblp.org/rec/conf/naacl/AndreasKL18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@misc{Kapelyukh2022-dall-e-bot,

title={DALL-E-Bot: Introducing Web-Scale Diffusion Models to Robotics},

author={Kapelyukh, Ivan and Vosylius, Vitalis and Johns, Edward},

publisher = {arXiv},

year={2022}

}


@inproceedings{Gammell2014-informedrrtstar,
  author    = {Jonathan D. Gammell and
               Siddhartha S. Srinivasa and
               Timothy D. Barfoot},
  title     = {Informed RRT*: Optimal sampling-based path planning focused via direct
               sampling of an admissible ellipsoidal heuristic},
  booktitle = {2014 {IEEE/RSJ} International Conference on Intelligent Robots and
               Systems, Chicago, IL, USA, September 14-18, 2014},
  pages     = {2997--3004},
  publisher = {{IEEE}},
  year      = {2014},
  url       = {https://doi.org/10.1109/IROS.2014.6942976},
  doi       = {10.1109/IROS.2014.6942976},
  timestamp = {Wed, 16 Oct 2019 14:14:51 +0200},
  biburl    = {https://dblp.org/rec/conf/iros/GammellSB14.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@misc{ni2022-ntfields,
  doi = {10.48550/ARXIV.2210.00120},
  
  url = {https://arxiv.org/abs/2210.00120},
  
  author = {Ni, Ruiqi and Qureshi, Ahmed H.},
  
  keywords = {Robotics (cs.RO), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {NTFields: Neural Time Fields for Physics-Informed Robot Motion Planning},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@inproceedings{liu2022regdeepdf,
  author =		 "Liu, P. and  Zhang, K. and Tateo D. and  Jauhri S. and  Peters J. and  Chalvatzaki G. and ",
  year =		 "2022",
  title =		 "Regularized Deep Signed Distance Fields for Reactive Motion Generation",
  booktitle =		 "2022 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)",
  URL =			 "https://www.ias.informatik.tu-darmstadt.de/uploads/Team/PuzeLiu/IROS_2022_ReDSDF.pdf",
}



@inproceedings{Ortiz2022-isdf,
  title={iSDF: Real-Time Neural Signed Distance Fields for Robot Perception},
  author={Ortiz, Joseph and Clegg, Alexander and Dong, Jing and Sucar, Edgar and Novotny, David and Zollhoefer, Michael and Mukadam, Mustafa},
  booktitle={Robotics: Science and Systems},
  year={2022}
}


@misc{liu2022atacomsdf,
  doi = {10.48550/ARXIV.2209.13308},
  
  url = {https://arxiv.org/abs/2209.13308},
  
  author = {Liu, Puze and Zhang, Kuo and Tateo, Davide and Jauhri, Snehal and Hu, Zhiyuan and Peters, Jan and Chalvatzaki, Georgia},
  
  keywords = {Robotics (cs.RO), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Safe reinforcement learning of dynamic high-dimensional robotic tasks: navigation, manipulation, interaction},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{finean2020compositesdf,
  author    = {Mark Nicholas Finean and
               Wolfgang Merkt and
               Ioannis Havoutis},
  editor    = {Susanne Biundo and
               Minh Do and
               Robert Goldman and
               Michael Katz and
               Qiang Yang and
               Hankz Hankui Zhuo},
  title     = {Predicted Composite Signed-Distance Fields for Real-Time Motion Planning
               in Dynamic Environments},
  booktitle = {Proceedings of the Thirty-First International Conference on Automated
               Planning and Scheduling, {ICAPS} 2021, Guangzhou, China (virtual),
               August 2-13, 2021},
  pages     = {616--624},
  publisher = {{AAAI} Press},
  year      = {2021},
  url       = {https://ojs.aaai.org/index.php/ICAPS/article/view/16010},
  timestamp = {Thu, 05 Aug 2021 14:31:51 +0200},
  biburl    = {https://dblp.org/rec/conf/aips/FineanMH21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}



@INPROCEEDINGS{Saulnier2020-infotheoreicalactiveexplorationsdf,
author={Saulnier, Kelsey and Atanasov, Nikolay and Pappas, George J. and Kumar, Vijay},  booktitle={2020 IEEE International Conference on Robotics and Automation (ICRA)},   title={Information Theoretic Active Exploration in Signed Distance Fields},   year={2020},  volume={},  number={},  pages={4080-4085},  doi={10.1109/ICRA40945.2020.9196882}}


@inproceedings{Li2022-implicitenvironmentfields,
  author    = {Xueting Li and
               Shalini De Mello and
               Xiaolong Wang and
               Ming{-}Hsuan Yang and
               Jan Kautz and
               Sifei Liu},
  title     = {Learning Continuous Environment Fields via Implicit Functions},
  booktitle = {The Tenth International Conference on Learning Representations, {ICLR}
               2022, Virtual Event, April 25-29, 2022},
  publisher = {OpenReview.net},
  year      = {2022},
  url       = {https://openreview.net/forum?id=3ILxkQ7yElm},
  timestamp = {Sat, 20 Aug 2022 01:15:42 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/LiMW0KL22.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@article{maken2022steinparticlefilter,
  author    = {Fahira Afzal Maken and
               Fabio Ramos and
               Lionel Ott},
  title     = {Stein Particle Filter for Nonlinear, Non-Gaussian State Estimation},
  journal   = {CoRR},
  volume    = {abs/2202.04213},
  year      = {2022},
  url       = {https://arxiv.org/abs/2202.04213},
  eprinttype = {arXiv},
  eprint    = {2202.04213},
  timestamp = {Fri, 18 Feb 2022 12:23:53 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2202-04213.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@misc{luo2022understandingdiffusionmodels,
  doi = {10.48550/ARXIV.2208.11970},
  
  url = {https://arxiv.org/abs/2208.11970},
  
  author = {Luo, Calvin},
  
  keywords = {Machine Learning (cs.LG), Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Understanding Diffusion Models: A Unified Perspective},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}




@misc{liu2022structdiffusion,
  doi = {10.48550/ARXIV.2211.04604},
  
  url = {https://arxiv.org/abs/2211.04604},
  
  author = {Liu, Weiyu and Hermans, Tucker and Chernova, Sonia and Paxton, Chris},
  
  keywords = {Robotics (cs.RO), Artificial Intelligence (cs.AI), Computation and Language (cs.CL), Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {StructDiffusion: Object-Centric Diffusion for Semantic Rearrangement of Novel Objects},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@inproceedings{watson22corl,
  author =		 "Watson, J. and  Peters, J.",
  year =		 "2022",
  title =		 "Inferring Smooth Control: Monte Carlo Posterior Policy Iteration with Gaussian Processes",
  booktitle =		 "Conference on Robot Learning",
  URL =			 "https://www.ias.informatik.tu-darmstadt.de/uploads/Team/JoeWatson/watson22corl.pdf",
}


@misc{johnson2021motionplanningtransformers,
  doi = {10.48550/ARXIV.2106.02791},
  
  url = {https://arxiv.org/abs/2106.02791},
  
  author = {Johnson, Jacob J. and Kalra, Uday S. and Bhatia, Ankit and Li, Linjun and Qureshi, Ahmed H. and Yip, Michael C.},
  
  keywords = {Robotics (cs.RO), Artificial Intelligence (cs.AI), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Motion Planning Transformers: A Motion Planning Framework for Mobile Robots},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


@article{Li2021mpc_mpnet,
  author    = {Linjun Li and
               Yinglong Miao and
               Ahmed Hussain Qureshi and
               Michael C. Yip},
  title     = {MPC-MPNet: Model-Predictive Motion Planning Networks for Fast, Near-Optimal
               Planning Under Kinodynamic Constraints},
  journal   = {{IEEE} Robotics Autom. Lett.},
  volume    = {6},
  number    = {3},
  pages     = {4496--4503},
  year      = {2021},
  url       = {https://doi.org/10.1109/LRA.2021.3067847},
  doi       = {10.1109/LRA.2021.3067847},
  timestamp = {Thu, 29 Apr 2021 15:11:56 +0200},
  biburl    = {https://dblp.org/rec/journals/ral/LiMQY21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@misc{qureshi2020cmpnetx,
  doi = {10.48550/ARXIV.2010.08707},
  
  url = {https://arxiv.org/abs/2010.08707},
  
  author = {Qureshi, Ahmed H. and Dong, Jiangeng and Baig, Asfiya and Yip, Michael C.},
  
  keywords = {Robotics (cs.RO), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), Differential Geometry (math.DG), FOS: Computer and information sciences, FOS: Computer and information sciences, FOS: Mathematics, FOS: Mathematics},
  
  title = {Constrained Motion Planning Networks X},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@misc{ajay2022decision_diffuser,
  doi = {10.48550/ARXIV.2211.15657},
  
  url = {https://arxiv.org/abs/2211.15657},
  
  author = {Ajay, Anurag and Du, Yilun and Gupta, Abhi and Tenenbaum, Joshua and Jaakkola, Tommi and Agrawal, Pulkit},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Is Conditional Generative Modeling all you need for Decision-Making?},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}





@inproceedings{Bhardwaj2020diffgpmp,
  author    = {Mohak Bhardwaj and
               Byron Boots and
               Mustafa Mukadam},
  title     = {Differentiable Gaussian Process Motion Planning},
  booktitle = {2020 {IEEE} International Conference on Robotics and Automation, {ICRA}
               2020, Paris, France, May 31 - August 31, 2020},
  pages     = {10598--10604},
  publisher = {{IEEE}},
  year      = {2020},
  url       = {https://doi.org/10.1109/ICRA40945.2020.9197260},
  doi       = {10.1109/ICRA40945.2020.9197260},
  timestamp = {Mon, 28 Sep 2020 12:19:28 +0200},
  biburl    = {https://dblp.org/rec/conf/icra/BhardwajBM20.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{
anonymous2023imitating,
title={Imitating Human Behaviour with Diffusion Models},
author={Anonymous},
booktitle={Submitted to The Eleventh International Conference on Learning Representations },
year={2023},
url={https://openreview.net/forum?id=Pv1GPQzRrC8},
note={under review}
}


@misc{huang2023scenediffuser,
  doi = {10.48550/ARXIV.2301.06015},
  
  url = {https://arxiv.org/abs/2301.06015},
  
  author = {Huang, Siyuan and Wang, Zan and Li, Puhao and Jia, Baoxiong and Liu, Tengyu and Zhu, Yixin and Liang, Wei and Zhu, Song-Chun},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Diffusion-based Generation, Optimization, and Planning in 3D Scenes},
  
  publisher = {arXiv},
  
  year = {2023},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@inproceedings{carvalho2022conditionedsbm,
  author    = {Carvalho, J. and  Baierl, M and  Urain, J and  Peters, J.},
  title     = {Conditioned Score-Based Models for Learning Collision-Free Trajectory Generation},
  booktitle = {NeurIPS 2022 Workshop on Score-Based Methods},
  year      = {2022},
}


@inproceedings{nichol2021improvedddpm,
  author    = {Alexander Quinn Nichol and
               Prafulla Dhariwal},
  editor    = {Marina Meila and
               Tong Zhang},
  title     = {Improved Denoising Diffusion Probabilistic Models},
  booktitle = {Proceedings of the 38th International Conference on Machine Learning,
               {ICML} 2021, 18-24 July 2021, Virtual Event},
  series    = {Proceedings of Machine Learning Research},
  volume    = {139},
  pages     = {8162--8171},
  publisher = {{PMLR}},
  year      = {2021},
  url       = {http://proceedings.mlr.press/v139/nichol21a.html},
  timestamp = {Wed, 25 Aug 2021 17:11:17 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/NicholD21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Dhariwal2021diffusionbeatsgans,
  author    = {Prafulla Dhariwal and
               Alexander Quinn Nichol},
  editor    = {Marc'Aurelio Ranzato and
               Alina Beygelzimer and
               Yann N. Dauphin and
               Percy Liang and
               Jennifer Wortman Vaughan},
  title     = {Diffusion Models Beat GANs on Image Synthesis},
  booktitle = {Advances in Neural Information Processing Systems 34: Annual Conference
               on Neural Information Processing Systems 2021, NeurIPS 2021, December
               6-14, 2021, virtual},
  pages     = {8780--8794},
  year      = {2021},
  url       = {https://proceedings.neurips.cc/paper/2021/hash/49ad23d1ec9fa4bd8d77d02681df5cfa-Abstract.html},
  timestamp = {Tue, 03 May 2022 16:20:47 +0200},
  biburl    = {https://dblp.org/rec/conf/nips/DhariwalN21.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Sohl-Dickstein2015diffusion,
  author    = {Jascha Sohl{-}Dickstein and
               Eric A. Weiss and
               Niru Maheswaranathan and
               Surya Ganguli},
  editor    = {Francis R. Bach and
               David M. Blei},
  title     = {Deep Unsupervised Learning using Nonequilibrium Thermodynamics},
  booktitle = {Proceedings of the 32nd International Conference on Machine Learning,
               {ICML} 2015, Lille, France, 6-11 July 2015},
  series    = {{JMLR} Workshop and Conference Proceedings},
  volume    = {37},
  pages     = {2256--2265},
  publisher = {JMLR.org},
  year      = {2015},
  url       = {http://proceedings.mlr.press/v37/sohl-dickstein15.html},
  timestamp = {Wed, 29 May 2019 08:41:45 +0200},
  biburl    = {https://dblp.org/rec/conf/icml/Sohl-DicksteinW15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@INPROCEEDINGS{kuffner2000rrtconnect,
  author={Kuffner, J.J. and LaValle, S.M.},
  booktitle={Proceedings 2000 ICRA. Millennium Conference. IEEE International Conference on Robotics and Automation. Symposia Proceedings (Cat. No.00CH37065)}, 
  title={RRT-connect: An efficient approach to single-query path planning}, 
  year={2000},
  volume={2},
  number={},
  pages={995-1001 vol.2},
  doi={10.1109/ROBOT.2000.844730}}




@inproceedings{Hansel_IICRA_2023,
  author ={Hansel, K. and  Urain, J. and  Peters, J. and  Chalvatzaki, G.},
  year = {2023},
  title = {Hierarchical Policy Blending as Inference for Reactive Robot Control},
  booktitle = {2023 IEEE International Conference on Robotics and Automation (ICRA)},
  publisher = {IEEE}
}

@inproceedings{Le__2022,
  author = {Le, A. T. and  Hansel, K. and  Peters, J. and  Chalvatzaki, G.},
  year = {2022},
  title =    {Hierarchical Policy Blending As Optimal Transport},
  booktitle ={arXiv preprint arXiv:2212.01938}
}

@article{wang2021survey,
  title={A survey of learning-based robot motion planning},
  author={Wang, Jiankun and Zhang, Tianyi and Ma, Nachuan and Li, Zhaoting and Ma, Han and Meng, Fei and Meng, Max Q-H},
  journal={IET Cyber-Systems and Robotics},
  volume={3},
  number={4},
  pages={302--314},
  year={2021},
  publisher={Wiley Online Library}
}



@ARTICLE{Elbanhawi2014sampling,
  author={Elbanhawi, Mohamed and Simic, Milan},
  journal={IEEE Access}, 
  title={Sampling-Based Robot Motion Planning: A Review}, 
  year={2014},
  volume={2},
  number={},
  pages={56-77},
  doi={10.1109/ACCESS.2014.2302442}}



@inproceedings{Liu_IICRA_2023,
  author =		 "Liu, P. and  Zhang, K. and  Tateo, D. and  Jauhri, S. and  Hu, Z. and  Peters, J. Chalvatzaki, G.",
  year =		 "2023",
  title =		 "Safe Reinforcement Learning of Dynamic High-Dimensional Robotic Tasks: Navigation, Manipulation, Interaction",
  booktitle =		 "2023 IEEE International Conference on Robotics and Automation (ICRA)",
  URL =			 "https://arxiv.org/abs/2209.13308",
  publisher =		 "ieee",
}



@book{lynch2017modernrobotics,
title = "Modern Robotics: Mechanics, Planning, and Control",
author = "Lynch, {Kevin M} and Park, {Frank C.}",
year = "2017",
language = "English (US)",
isbn = "978-1107156302",
publisher = "Cambridge Univeristy Press",
}



@inproceedings{hauser2010fastsmoothing,
  added-at = {2014-08-21T00:00:00.000+0200},
  author = {Hauser, Kris K. and Ng-Thow-Hing, Victor},
  biburl = {https://www.bibsonomy.org/bibtex/2604232d579a3e659e65d862988e0bc9b/dblp},
  booktitle = {ICRA},
  ee = {http://dx.doi.org/10.1109/ROBOT.2010.5509683},
  interhash = {6f8ebad3eabd9eb0187adfa266d6e120},
  intrahash = {604232d579a3e659e65d862988e0bc9b},
  keywords = {dblp},
  pages = {2493-2498},
  publisher = {IEEE},
  timestamp = {2015-06-20T03:06:23.000+0200},
  title = {Fast smoothing of manipulator trajectories using optimal bounded-acceleration shortcuts.},
  url = {http://dblp.uni-trier.de/db/conf/icra/icra2010.html#HauserN10},
  year = 2010
}


@inproceedings{herbert2017fastrack,
  title={FaSTrack: A modular framework for fast and guaranteed safe motion planning},
  author={Herbert, Sylvia L and Chen, Mo and Han, SooJean and Bansal, Somil and Fisac, Jaime F and Tomlin, Claire J},
  booktitle={2017 IEEE 56th Annual Conference on Decision and Control (CDC)},
  pages={1517--1522},
  year={2017},
  organization={IEEE}
}

@inproceedings{petti2005safe,
  title={Safe motion planning in dynamic environments},
  author={Petti, St{\'e}phane and Fraichard, Thierry},
  booktitle={2005 IEEE/RSJ International Conference on Intelligent Robots and Systems},
  pages={2210--2215},
  year={2005},
  organization={IEEE}
}


@article{karaman2011sampling,
  title={Sampling-based algorithms for optimal motion planning},
  author={Karaman, Sertac and Frazzoli, Emilio},
  journal={The international journal of robotics research},
  volume={30},
  number={7},
  pages={846--894},
  year={2011},
  publisher={Sage Publications Sage UK: London, England}
}


@inproceedings{le2021learning,
  title={Learning forceful manipulation skills from multi-modal human demonstrations},
  author={Le, An T and Guo, Meng and van Duijkeren, Niels and Rozo, Leonel and Krug, Robert and Kupcsik, Andras G and B{\"u}rger, Mathias},
  booktitle={2021 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={7770--7777},
  year={2021},
  organization={IEEE}
}

@misc{dhariwal2021diffusion,
    title={Diffusion Models Beat GANs on Image Synthesis},
    author={Prafulla Dhariwal and Alex Nichol},
    year={2021},
    eprint={2105.05233},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}



@incollection{pytorch2019,
title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
booktitle = {Advances in Neural Information Processing Systems 32},
pages = {8024--8035},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {http://papers.neurips.cc/paper/9015-pytorch-an-imperative-style-high-performance-deep-learning-library.pdf}
}



@inproceedings{sohn2015cvae,
 author = {Sohn, Kihyuk and Lee, Honglak and Yan, Xinchen},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {C. Cortes and N. Lawrence and D. Lee and M. Sugiyama and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Learning Structured Output Representation using Deep Conditional Generative Models},
 url = {https://proceedings.neurips.cc/paper/2015/file/8d55a249e6baa5c06772297520da2051-Paper.pdf},
 volume = {28},
 year = {2015}
}

@article{sola2018micro,
  title={A micro Lie theory for state estimation in robotics},
  author={Sola, Joan and Deray, Jeremie and Atchuthan, Dinesh},
  journal={arXiv preprint arXiv:1812.01537},
  year={2018}
}

@inproceedings{rasmussen2003gaussian,
  title={Gaussian processes in machine learning},
  author={Rasmussen, Carl Edward},
  booktitle={Summer school on machine learning},
  pages={63--71},
  year={2003},
  organization={Springer}
}

@inproceedings{barfoot2014batch,
  title={Batch Continuous-Time Trajectory Estimation as Exactly Sparse Gaussian Process Regression.},
  author={Barfoot, Tim D and Tong, Chi Hay and S{\"a}rkk{\"a}, Simo},
  booktitle={Robotics: Science and Systems},
  volume={10},
  pages={1--10},
  year={2014},
  organization={Citeseer}
}

@misc{grathwohl2020mcmc,
    title={No MCMC for me: Amortized sampling for fast and stable training of energy-based models},
    author={Will Grathwohl and Jacob Kelly and Milad Hashemi and Mohammad Norouzi and Kevin Swersky and David Duvenaud},
    year={2020},
    eprint={2010.04230},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

